Evaluating the Disentanglement of Deep Generative Models through Manifold Topology

Learning disentangled representations is regarded as a fundamental task for improving the generalization, robustness, and interpretability of generative models. However, measuring disentanglement has been challenging and inconsistent, often dependent on an ad-hoc external model or specific to a certain dataset. To address this, we present a method for quantifying disentanglement that only uses the generative model, by measuring the topological similarity of conditional submanifolds in the learned representation. This method showcases both unsupervised and supervised variants. To illustrate the effectiveness and applicability of our method, we empirically evaluate several state-of-the-art models across multiple datasets. We find that our method ranks models similarly to existing methods. We make ourcode publicly available at https://github.com/stanfordmlgroup/disentanglement.

==> algo_old.tex <==
% \documentclass{article}
% \usepackage[utf8]{inputenc}

% \usepackage{array}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{amssymb}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{mathtools}

% \begin{document}


\begin{algorithm}[h]
\caption{Experiment summary: For a given generator $g$ with latent prior $\mathcal{P}$ that has $D_z$ latent dimensions and $n_d$ samples for each latent dimension $d \in D_z$, our experimental procedure identifies a similarity matrix $M$ with the score-maximizing $c$ biclusters and returns a score $\mu$. $RLT()$ corresponds to the RLT-generating procedure from the Geometry Score paper.
Alternatively, with real data we assume a dataset $\mathcal{D}$ with $n_d$ possible values for a factor of variation $d$. The variable `generated' corresponds to whether the barcodes are real or generated. 
% For example, we set $\mathcal{P} \coloneqq \mathcal{N}(0, I_{D_z})$, where $I_{D_z}$ is the identity matrix. We also replace iterating over $n_d$ by sampling $k \sim \mathcal{N}(0,1)$ 10 times. % When we generate barcodes from real data, we sample factors of variation corresponding to $z'$ from the dataset conditioned on each potential value in $n_d$.
}
\begin{algorithmic}
\STATE $N \gets 1000$ \COMMENT{number samples}
\IF{generated}
    \FOR{$i$ in $1:N$}
        \STATE Sample $z^{(i)} \sim \mathcal{P}$ \COMMENT{note: $z\in \mathbb{R}^{N\times D_z}$}
    \ENDFOR
\ENDIF

\FOR{latent dimension $d$ in $1:D_z$} 
    \FOR{$k$ in $1:n_d$}
        \IF{generated}
            \STATE $z' \gets copy(z)$
            % \STATE Set $z'_d \gets k$
            \STATE Set $z'_d \gets k \sim \mathcal{P}_d$
            \STATE Set $x \gets g(z'_d)$
        \ELSE{}
            \STATE Set $z'_d, x \gets sample(\mathcal{D}\vert d=k$)
        \ENDIF
        \STATE Compute $e_z \gets embedding(x)$ \COMMENT{e.g. using VGG16}
        \STATE Compute $rlt[d, k] \gets RLT(e_z, \gamma=1/128, L_0=1000, n=100)$
        \STATE Compute $WB[d] \gets W. Barycenter(rlt[d, k])$
    \ENDFOR
\ENDFOR


\FOR{$d_1$ in $1:D_z$}
    \FOR{$d_2$ in $1:D_z$}
        \STATE Compute $M[d_1, d_2] \gets W. Distance(WB[d_1], WB[d_2])$
    \ENDFOR
\ENDFOR

\FOR{$c$ in $1:D_z$}
    \STATE Apply spectral coclustering to matrix $M$ using $c$ biclusters
    \STATE Compute metric $\mu$ based on in-group and out-group variances
\ENDFOR
\STATE Select optimal $c$
\RETURN $M$, $c$, $\mu$
\end{algorithmic}
\end{algorithm}

% \end{document}


==> fig_wbary.tex <==
\begin{figure}[h]
\begin{center}
\centerline{
\includegraphics[width=1.2\columnwidth]{figures/wbary.pdf}
}
\caption{Comparison of topological signatures in dSprites derived from the Euclidean mean on the left (a) and (b)~\cite{khrulkov2018geometry} to our method of deriving them from taking the Wasserstein barycenters on the right (c) and (d). Notice visually that the Euclidean mean collapses geometric information, rendering the two topological signatures (a) and (b) more indistinct, while the Wasserstein barycenters exhibit much smoother distributions and construct distinct topological signatures for each factor, (c) and (d).}
\label{fig:bary_vis}
\end{center}
\end{figure}
